A Focused Sequent Calculus Framework for Proof Search in Pure Type Systems

Basic proof-search tactics in logic and type theory can be seen as the root-first applications of rules in an appropriate sequent calculus, preferably without the redundancies generated by permutation of rules. This paper addresses the issues of defining such sequent calculi for Pure Type Systems (PTS, which were originally presented in natural deduction style) and then organizing their rules for effective proof-search. We introduce the idea of Pure Type Sequent Calculus with meta-variables (PTSCalpha), by enriching the syntax of a permutation-free sequent calculus for propositional logic due to Herbelin, which is strongly related to natural deduction and already well adapted to proof-search. The operational semantics is adapted from Herbelin's and is defined by a system of local rewrite rules as in cut-elimination, using explicit substitutions. We prove confluence for this system. Restricting our attention to PTSC, a type system for the ground terms of this system, we obtain the Subject Reduction property and show that each PTSC is logically equivalent to its corresponding PTS, and the former is strongly normalising iff the latter is. We show how to make the logical rules of PTSC into a syntax-directed system PS for proof-search, by incorporating the conversion rules as in syntax-directed presentations of the PTS rules for type-checking. Finally, we consider how to use the explicitly scoped meta-variables of PTSCalpha to represent partial proof-terms, and use them to analyse interactive proof construction. This sets up a framework PE in which we are able to study proof-search strategies, type inhabitant enumeration and (higher-order) unification.

==> Common/Macros_Main.tex <==
%Miscellaneous========================

\long\def\ignore#1{\relax}

\newcommand\homedir{~}
\newcommand\figurefont{\fontsize{9}{11}}

\newcommand\struto{\raise6pt\hbox{\strut}}%
\newcommand\strutb{\raise-6pt\hbox{\strut}}%

\newcommand\upline{\hline\struto}
\newcommand\midline{\\[+4pt]\hline\struto}
\newcommand\mmidline{\\[+4pt]\hline\hline\struto}
\newcommand\downline{\\[+4pt]\hline}

%Floating figures WHERE I WANT====================
\renewcommand{\topfraction}{0.95}  % max fraction of floats at top
\renewcommand{\bottomfraction}{0.95}       % max fraction of floats at bottom
\renewcommand\floatpagefraction{.5}
\renewcommand\textfraction{0.1}   
\setcounter{totalnumber}{50}
\setcounter{topnumber}{50}
\setcounter{bottomnumber}{50}
\floatsep5pt  
\intextsep5pt 
\abovecaptionskip1pt
\belowcaptionskip2pt

%Footnote
\interfootnotelinepenalty=1000000000

\newtheorem{warning}{Notice}

%% Proof and end-of-proof (due to Paul Taylor)
\newcommand\pushright[1]{{              % set up
    \parfillskip=0pt            % so \par doesnt push \square to left
    \widowpenalty=1000000000         % so we dont break the page before \square
    \displaywidowpenalty=10000  % ditto
    \finalhyphendemerits=0      % TeXbook exercise 14.32
    %%
    %%                 horizontal
    \leavevmode                 % \nobreak means lines not pages
    \unskip                     % remove previous space or glue
    \nobreak                    % don't break lines
    \hfil                       % ragged right if we spill over
    \penalty50                  % discouragement to do so
    \hskip.2em                  % ensure some space
    \null                       % anchor following \hfill
    \hfill                      % push \square to right
    {#1}                        % the end-of-proof mark (or whatever)
    %%
    %%                   vertical
    \par}}                      % build paragraph

\newcommand{\qedsymbol}{$\Box$}

\newenvironment{preuve}{\noindent{\bf Proof: }}
{}

\newenvironment{proof}{\noindent{\bf Proof: }}
{\pushright{\qedsymbol}\penalty-700 \smallskip}

\renewcommand{\paragraph}[1]{\mbox{}\\{\bf \large #1}}

\newenvironment{ann}[3][{}]
{\begin{trivlist}\item[]%\hspace{\parindent}
    {\bf {{#2}~\ref{#3}\ #1}}} 
{%\hfill \rule{.2em}{.2em}
\end{trivlist}}

\newenvironment{compactlist}
{\begin{list}{$\bullet$}{\setlength{\topsep}{0.07in}\setlength{\itemsep}{0in}}}
{\end{list}}

\newenvironment{compactenumerate}
{\begin{enumerate}{$\bullet$}{\setlength{\topsep}{0.07in}\setlength{\itemsep}{0in}}}
{\end{enumerate}}

\newcommand\mybox[1]{\fbox{\vbox{#1}}}
%\newcommand\mycbox[1]{\fbox{\vbox{#1}}}
\newcommand\mycbox[1]{\begin{tabular}{|l|}\upline #1 \downline\end{tabular}}
%\newcommand\mycbox[1]{\fbox{\bgroup#1\egroup}}


%General====================================================
\newcommand\abs[1]{{\left\vert#1\right\vert}}        % val.absolue
\newcommand\mn[1]{{\overline{#1}}}                   % moyenne
\renewcommand\v[1]{{\overrightarrow{#1}}}            % vecteur
\newcommand\M[1]{{\mathcal{#1}}}                     % grandeurs molaires
\newcommand\ti[1]{\widetilde{#1}}
\newcommand\unif{\bigcap}
\newcommand\unit{\textsf{unit}}
\newcommand\imp{\triangleright}
\newcommand\sub{\subseteq}
\newcommand\N{\mathbb{N}}
\newcommand\corner[1]{\langle #1 \rangle}


%Prooftrees=================================================
%\def\infer#1#2#3{\[#1\justifies #2\using #3\]}
%\def\Infer#1#2#3{\[#1\Justifies #2\using #3\]}
\newcommand\infers[3]{\infer[#3]{#2}{#1}}
\newcommand\Infers[3]{\begin{prooftree}#1\Justifies #2\using #3\end{prooftree}}

%Maths======================================================
\newcommand\dom[1]{\textsf{Dom}{(#1)}}
\newcommand\card[1]{|#1|}
\newcommand\maxi{\textsf{max}}
\newcommand{\sm}{\setminus}
\newcommand{\es}{\emptyset}
\newcommand{\eqdef}{:=\ }
\newcommand{\sqin}{\textsf{\footnotesize{E}}}
\newcommand{\sqes}{\not{\mbox{\![\hspace{-0.02cm}]}}}

%Greek======================================================
\renewcommand\a{\alpha}
\renewcommand\b{\beta}
\newcommand\g{\gamma}
\renewcommand\d{\delta}
\renewcommand\l{\lambda}
%\newcommand\m{\mu}
\newcommand\clambda{\mbox{$\lambda\hspace{-5.4pt}\lambda$}}


\newcommand{\Gam}{\Gamma}
\newcommand{\Gm}{\mbox{$\Gamma$}}
\newcommand{\Lam}{\Lambda}
\newcommand{\Del}{\Delta}
\newcommand{\Ups}{\Upsilon}
\newcommand{\Om}{\Omega}
\newcommand{\Sig}{\Sigma}
\newcommand{\sig}{\sigma}
\newcommand{\cals}{{\mathcal S}}
\newcommand{\calf}{{\mathcal F}}





%Logical systems & Calculi==================================

\newcommand\NJ{\textsf{NJi}}
\newcommand\LJ{\textsf{LJ}}
\newcommand\LK{\textsf{LK}}
%\newcommand\LKmm{$\textsf{LK}_{\mu\tilde\mu}$}

\newcommand\Gzs{\textsf{G1}}
\newcommand\Gz{\textsf{G1ii}}
\newcommand\Giiis{\textsf{G3}}
\newcommand\Giii{\textsf{G3ii}}
\newcommand\Giiii{\Giii}
\newcommand\Gthree{\Giii}

\newcommand\LJT{\textsf{LJT}}
\newcommand\LJQ{\textsf{LJQ}}

\newcommand{\LJQp}{\ensuremath{\mathbf \LJQ^\prime}}

\newcommand\Giv{\textsf{G4ii}}
\newcommand\Gfour{\Giv}

\newcommand\lG{\l\textsf{G3}}
\newcommand\lGcf{\l\textsf{G3}^{\textsf{cf}}}
\renewcommand\S{\textsf{S}}

\newcommand\lb{$\overline{\lambda}$}
\newcommand\lbm{\overline{\lambda}}
\newcommand\lLJQ{$\l\LJQ$}
\newcommand\lLJQm{\l\LJQ}

\newcommand\lm{$\lambda\mu$}
\newcommand\Lm{$\overline{\lambda}\mu$}
\newcommand\Lmm{$\overline{\lambda}\mu\widetilde{\mu}$}

\newcommand\LI{$\lambda I$}
\newcommand\Li{\Lambda I}

\newcommand\lx{$\l${\textsf x}}

\newcommand\lxx{$\l${\textsf {xx}}}

\renewcommand\ll{\lambda \textsf{lxr}}
\newcommand\lle{\l{\textsf {lxr}}}
\newcommand\Ll{$\lambda$l\textsf{xr}}

\newcommand\lC{$\l_{\textsf C}$}
\newcommand\lV{$\l_{\textsf{V}}$}

\newcommand\mathFomega{F_\omega}
\newcommand\Fomega{\ifmmode\mathFomega\else$\mathFomega$\fi}
\newcommand\mathFomegaC{F_\omega^{\mathcal C}}
\newcommand\FomegaC{\ifmmode\mathFomegaC\else$\mathFomegaC$\fi}
\newcommand\mathDNE{\mathrm{DNE}}
\newcommand\DNE{\ifmmode\mathDNE\else$\mathDNE$\fi}

\newcommand\PTS{{\textsf{PTS}}}
\newcommand\PTSC{{\textsf{PTSC}}}

\newcommand\CoC{{\textsf{CoC}}}
\newcommand\Coq{{\textsf{Coq}}}
\newcommand\Lego{{\textsf{Lego}}}
\newcommand\CoS{{\textsf{CoS}}}

\newcommand\KSf{\textsf{KSf}}
\newcommand\SKSf{\textsf{SKSf}}

\newcommand\KSfl{{\textsf {KSfl}}}
\newcommand\SKSfl{{\textsf {SKSfl}}}

\newcommand\FA{{Formalism \textsf {A}}}
\newcommand\FB{{Formalism \textsf {B}}}

\newcommand\BurA{Bureaucracy {\textsf {A}}}
\newcommand\BurB{Bureaucracy {\textsf {B}}}

%Abbrev==================================================

\renewcommand{\iff}{if and only if}
\newcommand{\mand}{\mbox{ and }}
\newcommand{\ie}{i.e.\ }
\newcommand{\eg}{e.g.\ }
\newcommand{\cf}{cf.\ }
\newcommand{\etc}{etc.\ }
\newcommand{\wrt}{w.r.t.\ }
\newcommand{\resp}{resp.\ }
\newcommand{\ih}{\mbox{by i.h.}}

